Untainted Puncturing for Irregular Low-Density Parity-Check Codes

Puncturing is a well-known coding technique widely used for constructing rate-compatible codes. In this paper, we consider the problem of puncturing low-density parity-check codes and propose a new algorithm for intentional puncturing. The algorithm is based on the puncturing of untainted symbols, i.e. nodes with no punctured symbols within their neighboring set. It is shown that the algorithm proposed here performs better than previous proposals for a range of coding rates and short proportions of punctured symbols.

==> Makefile <==
all : puncturing.pdf

puncturing.pdf : puncturing.dvi
	dvipdf $^

puncturing.dvi : \
	puncturing.tex \
	puncturing.bib \
	abstract.tex \
	introduction.tex \
	notation.tex \
	properties.tex \
	algorithm.tex \
	results.tex \
	conclusions.tex \
	results/peg10000-awgn.ps \
	results/peg10000-bec.ps \
	results/peg10000-bsc.ps
	latex $<
	bibtex puncturing 
	latex $<
	latex $<

clean :
	rm -rf *.aux *.log *.bbl *.blg *~ puncturing.dvi puncturing.pdf

